A Picture is Worth 500 Labels: A Case Study of Demographic Disparities in Local Machine Learning Models for Instagram and TikTok

Mobile apps have embraced user privacy by moving their data processing to the user's smartphone. Advanced machine learning (ML) models, such as vision models, can now locally analyze user images to extract insights that drive several functionalities. Capitalizing on this new processing model of locally analyzing user images, we analyze two popular social media apps, TikTok and Instagram, to reveal (1) what insights vision models in both apps infer about users from their image and video data and (2) whether these models exhibit performance disparities with respect to demographics. As vision models provide signals for sensitive technologies like age verification and facial recognition, understanding potential biases in these models is crucial for ensuring that users receive equitable and accurate services. We develop a novel method for capturing and evaluating ML tasks in mobile apps, overcoming challenges like code obfuscation, native code execution, and scalability. Our method comprises ML task detection, ML pipeline reconstruction, and ML performance assessment, specifically focusing on demographic disparities. We apply our methodology to TikTok and Instagram, revealing significant insights. For TikTok, we find issues in age and gender prediction accuracy, particularly for minors and Black individuals. In Instagram, our analysis uncovers demographic disparities in the extraction of over 500 visual concepts from images, with evidence of spurious correlations between demographic features and certain concepts.

==> tables/instagram_facial_mean_var_manual_False.tex <==
\begin{table*}
\scriptsize
    \centering
\caption{Mean and variance of Instagram facial concepts scores on the overall generated dataset. Range is scaled to 0--100. The abbreviations stand for \textbf{A}sian, \textbf{B}lack, \textbf{I}ndian, or \textbf{W}hite; and \textbf{M}ale or \textbf{F}emale. \checkmark~indicates statistical significance, and \xmark~indicates no statistical significance. NaN means no samples are present in the dataset for this concept-demographic group pair.}
\begin{tabular}{lr@{\hspace{0.5em}}rr@{\hspace{0.5em}}rr@{\hspace{0.5em}}rr@{\hspace{0.5em}}rr@{\hspace{0.5em}}rr@{\hspace{0.5em}}rr@{\hspace{0.5em}}rr@{\hspace{0.5em}}rlll}
\toprule
 \multirow{2}{*}{\textbf{concept}} & \multicolumn{2}{c}{\textbf{AM}} & \multicolumn{2}{c}{\textbf{AF}} & \multicolumn{2}{c}{\textbf{BM}} & \multicolumn{2}{c}{\textbf{BF}} & \multicolumn{2}{c}{\textbf{IM}} & \multicolumn{2}{c}{\textbf{IF}} & \multicolumn{2}{c}{\textbf{WM}} & \multicolumn{2}{c}{\textbf{WF}} &  \multirow{2}{*}{\textbf{NH~\ref{nullhyp:allsexscores}}}& \multirow{2}{*}{\textbf{NH~\ref{nullhyp:allethnicityscores}}} & \multirow{2}{*}{\textbf{NH~\ref{nullhyp:alldemogscores}}}\\
 & mean & var & mean & var & mean & var & mean & var & mean & var & mean & var & mean & var & mean & var &  &  &  \\
\midrule
beard & 53.55 & 8.09 & 53.35 & 9.638 & 55.53 & 3.584 & 51.66 & 5.884 & 83.82 & 2.445 & 73.69 & 3.778 & 71.83 & 3.417 & 68.48 & 4.997 & \checkmark & \checkmark & \checkmark \\
blond & 6.645 & NaN & NaN & NaN & 12.41 & NaN & 60.46 & 2.828 & NaN & NaN & NaN & NaN & 32.69 & 7.045 & 71.68 & 1.976 & \checkmark & \xmark & \checkmark \\
blonde & 4.147 & NaN & NaN & NaN & 4.258 & NaN & 57.69 & 2.397 & NaN & NaN & NaN & NaN & 43.77 & 9.239 & 78.51 & 1.537 & \checkmark & \checkmark & \checkmark \\
braiding & 6.877 & 0.1365 & 12.76 & 0.5159 & 13.49 & 1.183 & 17.19 & 1.488 & 7.091 & 0.3182 & 2.993 & NaN & 12.4 & 1.254 & 5.954 & NaN & \xmark & \xmark & \xmark \\
eyeglasses & 89.01 & 1.211 & 78.3 & 2.637 & 71.38 & 3.379 & 69.72 & 3.232 & 89.07 & 1.484 & 75.27 & 3.22 & 88.03 & 1.218 & 83.83 & 1.313 & \checkmark & \checkmark & \checkmark \\
eyewear & 67.52 & 4.051 & 60.25 & 4.502 & 45.16 & 3.899 & 49.13 & 3.549 & 75.54 & 2.791 & 64.61 & 3.895 & 72.95 & 3.628 & 74.59 & 2.347 & \checkmark & \checkmark & \checkmark \\
hair & 29.41 & 1.207 & 42.03 & 1.196 & 23.91 & 0.6619 & 41.12 & 1.142 & 19.25 & 0.7032 & 34.49 & 1.097 & 32.17 & 0.9552 & 49.44 & 0.7643 & \checkmark & \checkmark & \checkmark \\
hair\_long & 11.2 & 1.126 & 37.48 & 1.974 & 11.88 & 2.028 & 41.04 & 2.792 & 12.65 & 1.272 & 43.32 & 2.342 & 11.55 & 1.033 & 41.9 & 1.441 & \checkmark & \checkmark & \checkmark \\
jewelry & 34.04 & 2.921 & 34.39 & 2.403 & 43.76 & 2.314 & 58.44 & 1.945 & 39.43 & 5.557 & 63.69 & 3.14 & 38.97 & 2.227 & 44.04 & 1.676 & \checkmark & \checkmark & \checkmark \\
sunglass & 73.34 & 3.608 & 57.69 & 4.588 & 50.69 & 6.086 & 59.13 & 4.738 & 77.06 & 2.651 & 65.42 & 4.009 & 85.89 & 1.281 & 74.02 & 3.364 & \checkmark & \checkmark & \checkmark \\
\bottomrule
\end{tabular}
\label{tab:}
\end{table*}

